Pretraining Without Attention

Transformers have been essential to pretraining success in NLP. While other architectures have been used, downstream accuracy is either significantly worse, or requires attention layers to match standard benchmarks such as GLUE. This work explores pretraining without attention by using recent advances in sequence routing based on state-space models (SSMs). Our proposed model, Bidirectional Gated SSM (BiGS), combines SSM layers with a multiplicative gating architecture that has been effective in simplified sequence modeling architectures. The model learns static layers that do not consider pair-wise interactions. Even so, BiGS is able to match BERT pretraining accuracy on GLUE and can be extended to long-form pretraining of 4096 tokens without approximation. Analysis shows that while the models have similar average accuracy, the approach has different inductive biases than BERT in terms of interactions and syntactic representations. All models from this work are available at https://github.com/jxiw/BiGS.

==> checklist.tex <==
\newpage

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section }%~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We do not foresee any such negative impact yet.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We submit an anonymous URL with the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We did as much as possible in the scope of the main paper. Further details are deferred to the supplement.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the numbers and figures quantifying the error bars and the standard deviation in additional experimental results.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We have cited the codebases uses and the competing baselines.}
  \item Did you mention the license of the assets?
    \answerYes{All the external codebases used by us has a MIT License.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We add our code using an anonymous URL.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> images/glue.tex <==
\subsection{GLUE}

\begin{table*}[t]
\centering 
\label{glue}
\begin{tabular}{lc|rrrrrrrr|r}
\toprule
               &  Arch / Route & MNLI & QNLI &  QQP & RTE  & SST-2 & MRPC & COLA &  STS-B & AVG \\
 &   & 393k & 105k & 364k & 2.5k &  67k  & 3.7k & 8.5k & 7k & \\ 
\midrule
&& \multicolumn{9}{c}{$\sim 1.1e^{10}$ Tokens / $\sim$ 350M Parameters}\\
\midrule
BERT & \textsc{stack} / \textsc{att}  & 83.3 & 90.2 & 87.9 & 79.4 & 91.7 & 91.1 & 60.5 & 88.9 & 84.1 \\ 
  & \textsc{stack} / \textsc{ssm} & 78.4 & 83.5 & 85.6 &  60.5 & 91.6 & 83.9 & 53.1 & 81.3  &  77.2 \\ 
  & \textsc{gated} / \textsc{att} &  82.5 & 88.5 & 87.5 & 74.0 & 91.3 & 89.5 & 60.7 & 86.4 & 82.6 \\ 
BiGS  & \textsc{gated} / \textsc{ssm} & 82.9 & 89.3 & 87.7 & 76.5 & 92.6 & 89.6 & 64.7 & 88.5 & 84.0 \\ 
\midrule
&& \multicolumn{9}{c}{$\sim 2.9e^{10}$ Tokens / $\sim$ 350M Parameters}\\
\midrule
BERT & \textsc{stack} / \textsc{att} & 84.7 & 90.9 & 88.3 & 82.1 & 93.2 & 92.4 & 61.4 & 89.6 & 85.3 \\ 
  & \textsc{stack} / \textsc{ssm}   & 80.1 & 86.5 & 87.2 &  65.6 & 92.3 &  86.5    & 56.5 &  83.4  & 79.8 \\ 
  & \textsc{gated} / \textsc{att}   & 83.4 & 90.3 & 87.6 & 74.7 & 92.3 & 90.5 & 62.5 & 88.2 & 83.7 \\ 
BiGS  & \textsc{gated} / \textsc{ssm} & 84.7 & 90.5 & 88.3 & 79.5 & 94.2 & 90.0 & 65.2 & 89.6 & 85.3 \\ 
\midrule
&& \multicolumn{9}{c}{Non-Attention Based Pretraining} \\
\midrule
CNN & \textsc{stack} /  \textsc{cnn} & $\sim$75 & - &  - & - & 92.2 & - & - & - & -\\
ELMo & \textsc{stack} / \textsc{rnn} & 68.6 & 71.2 & 84.3 & 53.4 & 91.5 & 70.5 & 44.1 & 82.3 & 68.7\\
FNet-L & \textsc{stack} / \textsc{fnet} & 78.0 & 85.0 & 85.0 & 69.0 & 94.0 & 88.0 & - & 84.0 & - \\
\midrule
&& \multicolumn{9}{c}{GLUE Test} \\
\midrule
BERT\textsubscript{LARGE} & \textsc{stack} /  \textsc{ssm} & & & & & & & & & \\ 
BiGS\textsubscript{LARGE}  & \textsc{gated} / \textsc{ssm} & & & & & & & & & \\ 
\bottomrule
\end{tabular}
\caption{GLUE Development Results. (Top) Comparison of different architectures and routing in a controlled setting~\cite{izsak2021train}. See Figure~\ref{fig:model:architectures} for details. For RTE, MRPC, and STS-B we fine-tune from the MNLI checkpoint following convention by ~\cite{izsak2021train}. We report accuracy for MNLI, QNLI, RTE, SST-2 and
F1 score for QQP, MRPC and Matthew’s correlation for CoLA and Spearman’s
correlation for STS-B. (Bottom) Reported comparable results for other non-attention-based pretraining models based on CNNs, LSTMs and FNet~\cite{DBLP:conf/naacl/PetersNIGCLZ18, tay2021pre,lee2021fnet,wang2018glue}}\label{tab:glue}
\end{table*}

% \noindent \textbf{Pretraining}.~

Table~\ref{tab:glue} shows the main results for different pretrained models on the GLUE benchmark. 
BiGS replicates the accuracy of BERT at both scale of tokens. This result demonstrates that, at this computational budget, a state-space model can replicate the accuracy of a pretrained transformer model. These results are significantly better than other non-attention based pretrained models \cite{tay2021pre,lee2021fnet}. 

% such as ELMo and the pretrained CNN model~\cite{DBLP:conf/naacl/PetersNIGCLZ18, tay2021pre}. 
% These models 230M parameters / 500k steps (CNN model pretrained parameters )....

Multiplicative gating is necessary to achieve this accuracy. Without gating, the stacked SSM achieves a significantly worse result\footnote{Interestingly, both \textsc{stack} / \textsc{ssm} and \textsc{stack} / \textsc{att} reach the similar perplexity (4.4 for the shorter experiments). Transformer seems to transfer better than SSM at this level.}. To check if this benefit comes primarily from the use of gating, we train an attention based model using the \textsc{gate} architecture; however we find that this model actually achieves worse results than BERT. 


% We train with batch size of 256 sequences (256
% sequences * 512 tokens = 128,000 tokens/batch)
% for 1,000,000 steps, which is approximately 40



==> images/model_pic.tex <==
      

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt  

\begin{figure*}[htb]\label{fig:model:architecture}
    \centering
    \resizebox{0.6\textwidth}{!}{

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,705); %set diagram left start at 0, and has height of 705

%Flowchart: Process [id:dp8986354336311719] 
\draw  [fill={rgb, 255:red, 249; green, 249; blue, 249 }  ,fill opacity=1 ] (7,4) -- (644,4) -- (644,694) -- (7,694) -- cycle ;
%Shape: Rectangle [id:dp3081693185014942] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (125,312) -- (195,312) -- (195,352) -- (125,352) -- cycle ;
%Shape: Rectangle [id:dp9707465317246919] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (505,313) -- (589,313) -- (589,353) -- (505,353) -- cycle ;
%Shape: Rectangle [id:dp18821977500303788] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (245,313) -- (315,313) -- (315,353) -- (245,353) -- cycle ;
%Shape: Rectangle [id:dp5593348157793543] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (372,314) -- (442,314) -- (442,354) -- (372,354) -- cycle ;
%Shape: Rectangle [id:dp5892084940843731] 
\draw  [fill={rgb, 255:red, 28; green, 248; blue, 133 }  ,fill opacity=1 ] (127,249) -- (197,249) -- (197,289) -- (127,289) -- cycle ;
%Shape: Rectangle [id:dp6908537139858084] 
\draw  [fill={rgb, 255:red, 28; green, 248; blue, 133 }  ,fill opacity=1 ] (512,250.5) -- (594,250.5) -- (594,290) -- (512,290) -- cycle ;
%Shape: Rectangle [id:dp956199744141524] 
\draw  [fill={rgb, 255:red, 28; green, 248; blue, 133 }  ,fill opacity=1 ] (244,249) -- (314,249) -- (314,289) -- (244,289) -- cycle ;
%Shape: Rectangle [id:dp8886426274775596] 
\draw  [fill={rgb, 255:red, 28; green, 248; blue, 133 }  ,fill opacity=1 ] (372,252) -- (442,252) -- (442,292) -- (372,292) -- cycle ;
%Shape: Rectangle [id:dp22609957279224946] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (276,579.5) -- (421,579.5) -- (421,637) -- (276,637) -- cycle ;
%Straight Lines [id:da08806460889956425] 
\draw    (348,666.5) -- (348,642.5) ;
\draw [shift={(348,640.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp8379493584453621] 
\draw   (257,532.17) .. controls (257,522.41) and (264.06,514.5) .. (272.77,514.5) .. controls (281.47,514.5) and (288.53,522.41) .. (288.53,532.17) .. controls (288.53,541.94) and (281.47,549.85) .. (272.77,549.85) .. controls (264.06,549.85) and (257,541.94) .. (257,532.17) -- cycle ;
%Shape: Sine Wave Form [id:dp34263826098201755] 
\draw   (257,532.17) .. controls (263.41,519.97) and (266.44,519.91) .. (272.76,532.17) .. controls (279.09,544.44) and (282.06,544.51) .. (288.53,532.17) ;
%Shape: Rectangle [id:dp5780302505264014] 
\draw   (46,65.49) -- (626,65.49) -- (626,492.5) -- (46,492.5) -- cycle ;
%Straight Lines [id:da02639195242487391] 
\draw    (346,578.5) -- (343.03,403.5) ;
\draw [shift={(343,401.5)}, rotate = 89.03] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Or [id:dp7685169967387444] 
\draw   (331,531.25) .. controls (331,522.55) and (337.49,515.5) .. (345.5,515.5) .. controls (353.51,515.5) and (360,522.55) .. (360,531.25) .. controls (360,539.95) and (353.51,547) .. (345.5,547) .. controls (337.49,547) and (331,539.95) .. (331,531.25) -- cycle ; \draw   (331,531.25) -- (360,531.25) ; \draw   (345.5,515.5) -- (345.5,547) ;
%Straight Lines [id:da6119545529932782] 
\draw    (288.53,532.17) -- (312,531.69) -- (333,531.25) ;
%Shape: Rectangle [id:dp09959989068285369] 
\draw   (89,196.5) -- (606,196.5) -- (606,399.5) -- (89,399.5) -- cycle ;
%Shape: Rectangle [id:dp7184208659081879] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (295,428.5) -- (398,428.5) -- (398,473.5) -- (295,473.5) -- cycle ;
%Shape: Rectangle [id:dp4749485775349924] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (272,130.5) -- (412,130.5) -- (412,174.5) -- (272,174.5) -- cycle ;
%Straight Lines [id:da31890973769027786] 
\draw    (340,198.5) -- (338.15,173.49) ;
\draw [shift={(338,171.5)}, rotate = 85.76] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Right Angle [id:dp7640811615478458] 
\draw   (344,485) -- (71.36,482.48) -- (69,95.5) ;
%Straight Lines [id:da19530150916737377] 
\draw    (69,95.5) -- (319.12,95.74) ;
\draw [shift={(321.12,95.75)}, rotate = 180.06] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Or [id:dp7099790573064697] 
\draw   (321.12,95.75) .. controls (321.12,87.05) and (327.61,80) .. (335.62,80) .. controls (343.63,80) and (350.12,87.05) .. (350.12,95.75) .. controls (350.12,104.44) and (343.63,111.5) .. (335.62,111.5) .. controls (327.61,111.5) and (321.12,104.44) .. (321.12,95.75) -- cycle ; \draw   (321.12,95.75) -- (350.12,95.75) ; \draw   (335.62,80) -- (335.62,111.5) ;
%Straight Lines [id:da9338101353375521] 
\draw    (336,131.5) -- (335.66,110.5) ;
\draw [shift={(335.62,108.5)}, rotate = 89.06] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10525147285345748] 
\draw    (336,88.5) -- (335.25,65.49) -- (335.01,34.5) ;
\draw [shift={(335,32.5)}, rotate = 89.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da0792949006312007] 
\draw    (196,332.5) -- (242,333.46) ;
\draw [shift={(244,333.5)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da11621006921283294] 
\draw    (317,332.5) -- (368,332.5) ;
\draw [shift={(370,332.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da37870773506566047] 
\draw    (444,332.5) -- (502,332.5) ;
\draw [shift={(504,332.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da32571974042742013] 
\draw    (511,268.5) -- (442,269.47) ;
\draw [shift={(440,269.5)}, rotate = 359.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da02512233414685161] 
\draw    (371,272.5) -- (315,272.5) ;
\draw [shift={(313,272.5)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da367157831290704] 
\draw    (242,271.5) -- (197,271.5) ;
\draw [shift={(195,271.5)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5826421477454413] 
\draw    (157,371.5) -- (156.08,349.5) ;
\draw [shift={(156,347.5)}, rotate = 87.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da765686156386884] 
\draw    (278,372.5) -- (278,353.5) ;
\draw [shift={(278,351.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da11696782570524267] 
\draw    (401,374.5) -- (401,355.5) ;
\draw [shift={(401,353.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7600863452273658] 
\draw    (541,371.5) -- (541,352.5) ;
\draw [shift={(541,350.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da44945715329830116] 
\draw    (126,378.5) .. controls (134.96,389.45) and (67.68,306.34) .. (148.77,291.22) ;
\draw [shift={(150,291)}, rotate = 170.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da8938711997068072] 
\draw    (251,379.5) .. controls (238.07,389.45) and (182.56,327.13) .. (243.08,281.68) ;
\draw [shift={(244,281)}, rotate = 143.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da9611168003987782] 
\draw    (378,371) .. controls (365.07,380.95) and (309.56,318.63) .. (370.08,273.18) ;
\draw [shift={(371,272.5)}, rotate = 143.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da8123641972790303] 
\draw    (513,373.5) .. controls (500.07,383.45) and (444.56,321.13) .. (505.08,275.68) ;
\draw [shift={(506,275)}, rotate = 143.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da8879880176909003] 
\draw    (155,310.5) .. controls (95.3,299.56) and (72.73,216.59) .. (144.41,215.76) ;
\draw [shift={(145.5,215.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da14170055640047297] 
\draw    (269,310.5) .. controls (209.3,299.56) and (193.16,216.34) .. (264.91,215.51) ;
\draw [shift={(266,215.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da4165373644094481] 
\draw    (400,309.5) .. controls (340.3,298.56) and (313.27,217.57) .. (384.91,216.76) ;
\draw [shift={(386,216.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da5900141294882217] 
\draw    (543,309.5) .. controls (483.3,298.56) and (457.76,216.58) .. (529.41,215.76) ;
\draw [shift={(530.5,215.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da22662303104929205] 
\draw    (159,250.5) -- (159,233.5) ;
\draw [shift={(159,231.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Or [id:dp2889672852991605] 
\draw   (144.5,215.75) .. controls (144.5,207.05) and (150.99,200) .. (159,200) .. controls (167.01,200) and (173.5,207.05) .. (173.5,215.75) .. controls (173.5,224.45) and (167.01,231.5) .. (159,231.5) .. controls (150.99,231.5) and (144.5,224.45) .. (144.5,215.75) -- cycle ; \draw   (144.5,215.75) -- (173.5,215.75) ; \draw   (159,200) -- (159,231.5) ;
%Flowchart: Or [id:dp943661415552455] 
\draw   (266,215.5) .. controls (266,206.8) and (272.49,199.75) .. (280.5,199.75) .. controls (288.51,199.75) and (295,206.8) .. (295,215.5) .. controls (295,224.2) and (288.51,231.25) .. (280.5,231.25) .. controls (272.49,231.25) and (266,224.2) .. (266,215.5) -- cycle ; \draw   (266,215.5) -- (295,215.5) ; \draw   (280.5,199.75) -- (280.5,231.25) ;
%Flowchart: Or [id:dp7825708277966152] 
\draw   (386,216.75) .. controls (386,208.05) and (392.49,201) .. (400.5,201) .. controls (408.51,201) and (415,208.05) .. (415,216.75) .. controls (415,225.45) and (408.51,232.5) .. (400.5,232.5) .. controls (392.49,232.5) and (386,225.45) .. (386,216.75) -- cycle ; \draw   (386,216.75) -- (415,216.75) ; \draw   (400.5,201) -- (400.5,232.5) ;
%Flowchart: Or [id:dp2959447876967265] 
\draw   (530.5,215.75) .. controls (530.5,207.05) and (536.99,200) .. (545,200) .. controls (553.01,200) and (559.5,207.05) .. (559.5,215.75) .. controls (559.5,224.45) and (553.01,231.5) .. (545,231.5) .. controls (536.99,231.5) and (530.5,224.45) .. (530.5,215.75) -- cycle ; \draw   (530.5,215.75) -- (559.5,215.75) ; \draw   (545,200) -- (545,231.5) ;
%Straight Lines [id:da33161607566302975] 
\draw    (280.5,252.25) -- (280.5,233.25) ;
\draw [shift={(280.5,231.25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9276020021472238] 
\draw    (400.5,253.5) -- (400.5,234.5) ;
\draw [shift={(400.5,232.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3763958183678311] 
\draw    (545,252.5) -- (545,233.5) ;
\draw [shift={(545,231.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (279,598) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Word Embedding}};
% Text Node
\draw (327,669) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Input}};
% Text Node
\draw (91,523) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {Position Embedding};
% Text Node
\draw (413,405) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Bidirectional S4 block}};
% Text Node
\draw (320,439) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {Norm};
% Text Node
\draw (286,142) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {Feed Forward};
% Text Node
\draw (309,5) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {Output};
% Text Node
\draw (127,324) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Forward}};
% Text Node
\draw (247,324) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Forward}};
% Text Node
\draw (373,325) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Forward}};
% Text Node
\draw (510,324) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Forward}};
% Text Node
\draw (512,261) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Backward}};
% Text Node
\draw (367,261) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Backward}};
% Text Node
\draw (239,262) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Backward}};
% Text Node
\draw (121,260) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Backward}};
% Text Node
\draw (134,371) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large [CLS]}};
% Text Node
\draw (519,372) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large [SEP]}};
% Text Node
\draw (270,372) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large w1}};
% Text Node
\draw (389,373) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large w2}};
% Text Node
\draw (10,277) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large N x}};


\end{tikzpicture}





}
\caption{An overview architecture of pretrained models based on SSM’s family. The pretrained model first takes into a sequence of tokens, up to 128. After passing through the word embedding layer and adding the positional embeddings, we applied the pre-layer norm. The Bidirectional S4 block is the core where we have two blocks of S4 for forward and backward purposes. The model concats feed-forward layer' output and the skip to obtain the (intermediate) output. }
\end{figure*}

